Stochastic Vision Transformers with Wasserstein Distance-Aware Attention

Self-supervised learning is one of the most promising approaches to acquiring knowledge from limited labeled data. Despite the substantial advancements made in recent years, self-supervised models have posed a challenge to practitioners, as they do not readily provide insight into the model's confidence and uncertainty. Tackling this issue is no simple feat, primarily due to the complexity involved in implementing techniques that can make use of the latent representations learned during pre-training without relying on explicit labels. Motivated by this, we introduce a new stochastic vision transformer that integrates uncertainty and distance awareness into self-supervised learning (SSL) pipelines. Instead of the conventional deterministic vector embedding, our novel stochastic vision transformer encodes image patches into elliptical Gaussian distributional embeddings. Notably, the attention matrices of these stochastic representational embeddings are computed using Wasserstein distance-based attention, effectively capitalizing on the distributional nature of these embeddings. Additionally, we propose a regularization term based on Wasserstein distance for both pre-training and fine-tuning processes, thereby incorporating distance awareness into latent representations. We perform extensive experiments across different tasks such as in-distribution generalization, out-of-distribution detection, dataset corruption, semi-supervised settings, and transfer learning to other datasets and tasks. Our proposed method achieves superior accuracy and calibration, surpassing the self-supervised baseline in a wide range of experiments on a variety of datasets.

==> chapters/past_edits.tex <==
\begin{table}
	\centering
		\begin{tabular}{c c c c }
        \hline
        {$\mathbf{\lambda_1}$} & { $\mathbf{\lambda_2}$} & {\bf Accuracy}($\uparrow$) &  \\
         \hline
         $1e^{-4}$ & $1e^{-4}$ & \textbf{69.420}\\
         $1e^{-3}$ & $1e^{-3}$ & 61.310 \\
         $1e^{-4}$ & $1e^{-3}$ & 60.460 \\
         $1e^{-3}$ & $1e^{-4}$ & 59.390 \\
         $1e^{-5}$ & $1e^{-5}$ & 51.160   \\
		\end{tabular}
  \end{table}




\begin{table}\caption[Augmentation Ablation]{Performance of Wasserstein attention transformers with differing augmentations magnitude, standard deviations, and amount. The augmentations are constructed with the RandAugment augmentation policy.} \label{tab:ablation-augmentations}
	\centering
		\begin{tabular}{c c c  }
        \hline
        Aug. Magnitude & No. Aug & {\bf Accuracy} ($\uparrow$) \\
         \hline
         9 & 2 &  69.420 \\
         9 & 4 & 58.780  \\
         9 & 1 &  \textbf{71.370 } \\
         10 & 2 & 66.560 \\
         6 & 2 &  70.920 \\
		\end{tabular}
  \end{table}
